Computing Lewis Weights to High Precision

We present an algorithm for computing approximate $\ell_p$ Lewis weights to high precision. Given a full-rank $\mathbf{A} \in \mathbb{R}^{m \times n}$ with $m \geq n$ and a scalar $p>2$, our algorithm computes $\epsilon$-approximate $\ell_p$ Lewis weights of $\mathbf{A}$ in $\widetilde{O}_p(\log(1/\epsilon))$ iterations; the cost of each iteration is linear in the input size plus the cost of computing the leverage scores of $\mathbf{D}\mathbf{A}$ for diagonal $\mathbf{D} \in \mathbb{R}^{m \times m}$. Prior to our work, such a computational complexity was known only for $p \in (0, 4)$ [CohenPeng2015], and combined with this result, our work yields the first polylogarithmic-depth polynomial-work algorithm for the problem of computing $\ell_p$ Lewis weights to high precision for all constant $p > 0$. An important consequence of this result is also the first polylogarithmic-depth polynomial-work algorithm for computing a nearly optimal self-concordant barrier for a polytope.

==> defs.tex <==

\newtheorem{claim}{Claim}
\newtheorem{remark}{Remark}[section]
\newtheorem{fact}{Fact}[section]



\makeatletter
\def\ALG@special@indent{%
    \ifdim\ALG@thistlm=0pt\relax
        \hskip-\leftmargin
    \else
        \hskip\ALG@thistlm
    \fi
}
\newcommand{\NoIndentInAlg}[1]{\item[]\noindent\ALG@special@indent \ #1}


\newcommand{\compresslist}{ %
\setlength{\itemsep}{1pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}} %
\newcommand{\tikzmark}[1]{\tikz[overlay,remember picture] \node (#1) {};}
\newcommand\encircle[1]{%
  \tikz[baseline=(X.base)] 
    \node (X) [draw, shape=circle, inner sep=0] {\strut #1};}

\newcommand*{\AddNote}[4]{%
    \begin{tikzpicture}[overlay, remember picture]
        \draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
            ($(#3)!(#1.north)!($(#3)-(0,1)$)$) --  
            ($(#3)!(#2.south)!($(#3)-(0,1)$)$)
                node [align=center, text width=2.5cm, pos=0.5, anchor=west] {#4};
    \end{tikzpicture}
}%

\newcommand*\numcircledtikz[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=1.2pt] (char) {#1};}} 
\global\long\def\defeq{\stackrel{\mathrm{{\scriptscriptstyle def}}}{=}} %


\newcommand{\inprod}[2]{\langle {#1} , {#2} \rangle}
\providecommand{\norm}[1][]{$\left\vert\kern-0.25ex\left\vert {}\cdot{} \right\vert\kern-0.25ex\right\vert \ifx\\#1\\\else\left\vert\kern-0.25ex\left\vert#1\right\vert\kern-0.25ex\right\vert\fi$}
\providecommand{\abs}[1]{$\vert #1 \vert$}
\newcommand{\threepartdef}[6]
{
	\left\{
		\begin{array}{lll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{if } #4 \\
			#5 & \mbox{ } #6
		\end{array}
	\right.
}
\newcommand{\twopartdef}[4]
{
	\left\{
		\begin{array}{lll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{ } #4 
		\end{array}
	\right.
}

\newcommand{\boldvec}[2]{\mathbf{#1}_{\mathbf{#2}}}


\newcommand{\eat}[1]{}
\newcommand{\hide}[1]{{\color{red}Contents hidden!}}
\newcommand{\ones}{\mathbf 1}
\newcommand{\1}{\mathbf{1}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\reals}{\mathbb{R}} %
\newcommand{\R}{\mathbb{R}}
\newcommand{\symm}{\mathbb{S}}  %
\newcommand{\diag}{\mathop{\mathbf{diag}}}
\newcommand{\Diag}{\mathop{\mathbf{Diag}}}
\newcommand{\nnz}[1]{\mathop{\mathbf{nnz}}(#1)}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\newcommand{\argmax}{\mathop{\mathrm{ argmax}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\beps}{\overline{\varepsilon}}
\newcommand{\teps}{\widetilde{\varepsilon}}

\newcommand{\gradA}{\mathcal{C}_{\textup{grad}}}
\newcommand{\ratioconst}{\gamma}
\newcommand{\sumrescaling}{\zeta}
\newcommand{\fobj}{\mathcal{F}}
\newcommand{\costCP}{\mathcal{T}_{\mathrm{CP}}} 
\newcommand{\costLevScores}{\mathcal{T}_{\mathrm{lev}}}
\newcommand{\costlinsys}{\mathcal{T}_{\mathrm{Ax=b}}}
\newcommand{\polyeps}{\text{poly}($1/\eps$) }

\newcommand{\mA}{\mathbf{A}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\mSigma}{\mathbf{\Sigma}}
\newcommand{\mDiag}{\mathbf{Diag}}
\newcommand{\mZero}{\mathbf{0}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\dir}{\mathcal{D}} %
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mMl}{\mathbf{M}_{w\leq \eta}}


\newcommand{\winit}{w_{\textup{init}}}
\newcommand{\ww}{\overline{w}}
\newcommand{\wmid}{\widetilde{w}}
\newcommand{\lw}{\overline{w}}
\newcommand{\heps}{\widehat{\eps}}
\newcommand{\hw}{\widehat{w}}
\newcommand{\wopt}{\lw} %

\newcommand{\mwopt}{\overline{\mW}} 
\newcommand{\mwinit}{\mW_{\textup{init}}}
\newcommand{\mwmid}{\mathbf{\widetilde{W}}}
\newcommand{\mWW}{\mathbf{\widehat{W}}}
\newcommand{\mWWl}{\mathbf{\widehat{W}}_{w\leq \eta}}
\newcommand{\mWWg}{\mathbf{\widehat{W}}_{w> \eta}} 
\newcommand{\mWl}{\mathbf{W}_{w\leq \eta}}
\newcommand{\mWg}{\mathbf{W}_{w>\eta}}
\newcommand{\wround}{w_{\textrm{R}}}
\newcommand{\mwround}{\mathbf{W}_{\textrm{R}}}

\newcommand{\tepsval}{\tfrac{\alpha^8 \eps^4}{(25 m (\sqrt{n} + \alpha)  (\alpha + \alpha^{-1}))^4}}
\newcommand{\alphamax}{\bar{\alpha}}
\newcommand{\Ord}{\mathcal{O}}
\newcommand{\zeros}{\mathbf{0}}
\newcommand{\Prog}{\text{Descent }}
\newcommand{\prog}{\text{descent }}
\newcommand{\corr}{\text{correctional }}
\newcommand{\Corr}{\text{Correctional }}
\newcommand{\step}{\text{progress step }}
\newcommand{\stepcode}{\textbf{Progress }}
\newcommand{\progcode}{\textbf{Descent}}
\newcommand{\round}{\text{round}}
\newcommand{\roundcode}{\textbf{Round}}
\newcommand{\roundparallelcode}{\textbf{RoundParallel}}
\newcommand{\roundsequentialcode}{\textbf{RoundSequential}}
\newcommand{\coordset}{\textup{C}}
\newcommand{\coordsetcode}{\textup{S}}
\newcommand{\seqalgcode}{\textbf{SequentialAlg}}
\newcommand{\seq}{\text{sequential }}
\newcommand{\nonprog}{\text{non-descent }}
\newcommand{\rescale}{\text{rescale }}
\newcommand{\Nonprog}{\text{Non-Descent }}
\newcommand{\totaliters}{\mathcal{T}_{\textrm{total}}}
\newcommand{\totalitersrp}{\mathcal{T}_{\textrm{round\_parallel}}}
\newcommand{\totalitersonestep}{\mathcal{T}_{\textrm{no\_rounding}}}
\newcommand{\vDiag}{\mathbf{diag}}
\newcommand{\termone}{\textrm{T}_1}
